Bayesian causal inference in automotive software engineering and online evaluation

Randomised field experiments, such as A/B testing, have long been the gold standard for evaluating software changes. In the automotive domain, running randomised field experiments is not always desired, possible, or even ethical. In the face of such limitations, we develop a framework BOAT (Bayesian causal modelling for ObvservAtional Testing), utilising observational studies in combination with Bayesian causal inference, in order to understand real-world impacts from complex automotive software updates and help software development organisations arrive at causal conclusions. In this study, we present three causal inference models in the Bayesian framework and their corresponding cases to address three commonly experienced challenges of software evaluation in the automotive domain. We develop the BOAT framework with our industry collaborator, and demonstrate the potential of causal inference by conducting empirical studies on a large fleet of vehicles. Moreover, we relate the causal assumption theories to their implications in practise, aiming to provide a comprehensive guide on how to apply the causal models in automotive software engineering. We apply Bayesian propensity score matching for producing balanced control and treatment groups when we do not have access to the entire user base, Bayesian regression discontinuity design for identifying covariate dependent treatment assignments and the local treatment effect, and Bayesian difference-in-differences for causal inference of treatment effect overtime and implicitly control unobserved confounding factors. Each one of the demonstrative case has its grounds in practise, and is a scenario experienced when randomisation is not feasible. With the BOAT framework, we enable online software evaluation in the automotive domain without the need of a fully randomised experiment.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> chapters/app1.tex <==
\section*{Appendix A}

\begin{table*}[t]
\caption{Descriptive statistics of the target variable and covariates as inputs to Bayesian propensity score matching model, and a description of how the variables are computed. Each variable is aggregated to the vehicle level and max-min scaled.}
\centering
\begin{tabular}{lllll}
%{p{0.2\linewidth}p{0.5\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
\textbf{Variables} & \textbf{Variable description} & \textbf{Group} & \textbf{Mean} & \textbf{Std.} \\ \hline\hline
\textbf{Target variable} &  &  &  &  \\
\multirow{2}{*}{Fuel consumption {[}g/km{]}} & \multirow{2}{*}{total fuel injected in engine / total distance} & Control & 0.391 & 0.155 \\
 &  & Treatment & 0.354 & 0.123 \\ \hline
\textbf{Covariates} &  &  &  &  \\
\multirow{2}{*}{Share of trip start at a high state-of-charge} & \multirow{2}{*}{number of trip where soc\_start \textgreater 80\%} & Control & 0.356 & 0.177 \\
 &  & Treatment & 0.397 & 0.178 \\
\multirow{2}{*}{Share of trip end at a low state-of-charge} & \multirow{2}{*}{number of trip where soc\_end \textless 21\%} & Control & 0.258 & 0.155 \\
 &  & Treatment & 0.120 & 0.150 \\
\multirow{2}{*}{Number of trips made on weekdays} & \multirow{2}{*}{number of trips taken place during weekdays} & Control & 0.290 & 0.167 \\
 &  & Treatment & 0.225 & 0.153 \\
\multirow{2}{*}{Number of trips made on weekends} & \multirow{2}{*}{number of trips taken place during weekends} & Control & 0.269 & 0.173 \\
 &  & Treatment & 0.190 & 0.154 \\
\multirow{2}{*}{Average trip distance {[}km{]}} & \multirow{2}{*}{total trip distance / total number of trips} & Control & 0.301 & 0.132 \\
 &  & Treatment & 0.343 & 0.124 \\
\multirow{2}{*}{Maximum trip distance {[}km{]}} & \multirow{2}{*}{longest trip occurred during the observation period} & Control & 0.278 & 0.193 \\
 &  & Treatment & 0.240 & 0.186 \\
\multirow{2}{*}{Average trip speed {[}km/h{]}} & \multirow{2}{*}{total trip distance / total trip duration} & Control & 0.575 & 0.110 \\
 &  & Treatment & 0.624 & 0.117 \\
\multirow{2}{*}{Maximum trip speed {[}km/h{]}} & \multirow{2}{*}{highest trip speed occurred during the observation period} & Control & 0.637 & 0.125 \\
 &  & Treatment & 0.640 & 0.135 \\
\multirow{2}{*}{Share of distance on "hybrid"} & \multirow{2}{*}{distance driven when vehicle is in hybrid mode / total distance} & Control & 0.956 & 0.103 \\
 &  & Treatment & 0.987 & 0.033 \\
\multirow{2}{*}{Share of trips with a trailer attached} & \multirow{2}{*}{numbers of trip with trailer attached / total number of trips} & Control & 0.034 & 0.081 \\
 &  & Treatment & 0.034 & 0.075 \\
\multirow{2}{*}{Average number of engine starts in a trip} & \multirow{2}{*}{total occurrence of engine RPM \textgreater 500 / total number of trips} & Control & 0.169 & 0.112 \\
 &  & Treatment & 0.176 & 0.176 \\
\multirow{2}{*}{Average ambient temperature {[}$^\circ C${]}} & \multirow{2}{*}{average temperature measured at car during the period} & Control & 0.371 & 0.084 \\
 &  & Treatment & 0.372 & 0.071 \\
\multirow{2}{*}{Minimum ambient temperature {[}$^\circ C${]}} & \multirow{2}{*}{minimum temperature measure at car during the period} & Control & 0.497 & 0.135 \\
 &  & Treatment & 0.563 & 0.150 \\
\multirow{2}{*}{Maximum ambient temperature {[}$^\circ C${]}} & \multirow{2}{*}{maximum temperature measure at car during the period} & Control & 0.388 & 0.101 \\
 &  & Treatment & 0.374 & 0.099 \\ \hline
\end{tabular}
\label{table_data_bpsm}
\end{table*}


